CMT: A Memory Compression Method for Continual Knowledge Learning of Large Language Models

Large Language Models (LLMs) need to adapt to the continuous changes in data, tasks, and user preferences. Due to their massive size and the high costs associated with training, LLMs are not suitable for frequent retraining. However, updates are necessary to keep them in sync with rapidly evolving human knowledge. To address these challenges, this paper proposes the Compression Memory Training (CMT) method, an efficient and effective online adaptation framework for LLMs that features robust knowledge retention capabilities. Inspired by human memory mechanisms, CMT compresses and extracts information from new documents to be stored in a memory bank. When answering to queries related to these new documents, the model aggregates these document memories from the memory bank to better answer user questions. The parameters of the LLM itself do not change during training and inference, reducing the risk of catastrophic forgetting. To enhance the encoding, retrieval, and aggregation of memory, we further propose three new general and flexible techniques, including memory-aware objective, self-matching and top-aggregation. Extensive experiments conducted on three continual learning datasets (i.e., StreamingQA, SQuAD and ArchivalQA) demonstrate that the proposed method improves model adaptability and robustness across multiple base LLMs (e.g., +4.07 EM & +4.19 F1 in StreamingQA with Llama-2-7b).

==> checklist.tex <==
\clearpage
% 本论文：

% 包括介绍所使用AI方法的概念框架和/或伪代码描述（是/部分/否/不适用）
% 清晰区分意见、假设和推测与客观事实和结果（是/否）
% 为不太熟悉的读者提供清晰标记的教学参考，以获取复制论文所需的背景知识（是/否）
% 这篇论文是否有理论贡献？（是/否）

% 如果是，请完成以下列表。

% 清楚且正式地陈述所有假设和限制。（是/部分/否）
% 正式陈述所有新颖的主张（例如，在定理陈述中）。（是/部分/否）
% 包括所有新颖主张的证明。（是/部分/否）
% 为复杂和/或新颖的结果提供证明概述或直观解释。（是/部分/否）
% 对所用理论工具进行适当引用。（是/部分/否）
% 所有理论主张都通过实验证明成立。（是/部分/否/不适用）
% 所有用来否定或推翻主张的实验代码都包括在内。（是/否/不适用）
% 这篇论文是否依赖一个或多个数据集？（是/否）

% 如果是，请完成以下列表。

% 解释为什么在选定数据集上进行实验的动机。（是/部分/否/不适用）
% 所有在论文中引入的新数据集都包括在数据附录中。（是/部分/否/不适用）
% 所有在论文中引入的新数据集将在论文发表时公开，允许研究用途的免费使用许可。（是/部分/否/不适用）
% 所有来自现有文献的数据集（可能包括作者之前发表的工作）都附有适当的引用。（是/否/不适用）
% 所有来自现有文献的数据集都是公开的。（是/部分/否/不适用）
% 所有未公开的数据集都进行了详细描述，并解释了为什么公开的替代方案在科学上不够令人满意。（是/部分/否/不适用）
% 这篇论文是否包括计算实验？（是/否）

% 如果是，请完成以下列表。


\section{Reproducibility Checklist}
This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced \answerYes
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. \answerYes
\vspace{-4mm}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \answerYes
\end{itemize}

\noindent Does this paper make theoretical contributions? \answerNo


\noindent If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\noindent  Does this paper rely on one or more datasets? \answerYes

\noindent  If yes, please complete the list below.

\begin{itemize}
   
 \item A motivation is given for why the experiments are conducted on the selected datasets \answerYes
 \item All novel datasets introduced in this paper are included in a data appendix. \answerNA
 \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerNA
 \vspace{-4mm}
 \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes
 \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerNA
\end{itemize}

\noindent  Does this paper include computational experiments? \answerYes

\noindent  If yes, please complete the list below.
\begin{itemize}
 \item Any code required for pre-processing data is included in the appendix. \answerNo
 \item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerNo
 \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes
 \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \answerYes
 \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerYes
 \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes
 \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes
 \item This paper states the number of algorithm runs used to compute each reported result. \answerYes
 \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes
 \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \answerNo
 \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes
 \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes
\end{itemize}

% 任何用于数据预处理的代码都包括在附录中。（是/部分/否）
% 所有用于进行和分析实验的源代码都包括在代码附录中。（是/部分/否）
% 所有用于进行和分析实验的源代码将在论文发表时公开，并允许研究用途的免费使用许可。（是/部分/否）
% 所有实现新方法的源代码都有详细的注释，并引用论文中每一步的出处。（是/部分/否）
% 如果算法依赖随机性，则描述用于设置种子的方法，以便足以复制结果。（是/部分/否/不适用）
% 本文描述了用于运行实验的计算基础设施（硬件和软件），包括GPU/CPU型号、内存量、操作系统、相关软件库和框架的名称和版本。（是/部分/否）
% 本文正式描述了评估指标，并解释了选择这些指标的动机。（是/部分/否）
% 本文说明了用于计算每个报告结果的算法运行次数。（是/否）
% 实验分析不仅限于性能的单维度总结（例如，平均值；中位数），还包括变化、置信度或其他分布信息的度量。（是/否）
% 任何性能提升或下降的显著性都使用适当的统计检验方法进行评估（例如，Wilcoxon符号秩检验）。（是/部分/否）
% 本文列出了实验中每个模型/算法的所有最终（超）参数。（是/部分/否/不适用）
% 本文说明了在论文开发过程中尝试的每个（超）参数的数量和范围，以及选择最终参数设置的标准。（是/部分/否/不适用）
